Computational Approaches for Stochastic Shortest Path on Succinct MDPs

We consider the stochastic shortest path (SSP) problem for succinct Markov decision processes (MDPs), where the MDP consists of a set of variables, and a set of nondeterministic rules that update the variables. First, we show that several examples from the AI literature can be modeled as succinct MDPs. Then we present computational approaches for upper and lower bounds for the SSP problem: (a)~for computing upper bounds, our method is polynomial-time in the implicit description of the MDP; (b)~for lower bounds, we present a polynomial-time (in the size of the implicit description) reduction to quadratic programming. Our approach is applicable even to infinite-state MDPs. Finally, we present experimental results to demonstrate the effectiveness of our approach on several classical examples from the AI literature.

==> preliminaries_arxiv.tex <==
\section{Preliminaries}





\noindent{\bf Characteristic Random Variables.} Given random variables $X_0,\dots,X_n$ from a probability space $(\Omega,\mathcal{F},\probm)$ and a predicate $\Phi$ over $\Rset \cup \{-\infty,+\infty\}$, we denote by $\mathbf{1}_{\Phi(X_0,\dots,X_n)}$ the random variable such that
$\mathbf{1}_{\Phi(X_0,\dots,X_n)}(\omega)=1$ if $\Phi\left(X_0(\omega),\dots,X_n(\omega)\right)$ holds, and
$\mathbf{1}_{\Phi(X_0,\dots,X_n)}(\omega)=0$ otherwise.
%\[
%\mathbf{1}_{\Phi(X_0,\dots,X_n)}(\omega)=
%\begin{cases}
%1 & \mbox{if }\Phi\left(X_0(\omega),\dots,X_n(\omega)\right)\mbox{ holds} \\
%0 & \mbox{otherwise}
%\end{cases}\enskip.
%\]
By definition, $\expv\left(\mathbf{1}_{\Phi(X_0,\dots,X_n)}\right)=\probm\left(\Phi(X_0,\dots,X_n)\right)$.
%\begin{eqnarray*}
%\expv\left(\mathbf{1}_{\Phi(X_0,\dots,X_n)}\right)&=&1\cdot \probm\left(\{\omega\mid \Phi(X_0(\omega),\dots,X_n(\omega))\}\right)\\
%&=& \probm\left(\Phi(X_0,\dots,X_n)\right)~~.
%\end{eqnarray*}
Note that if $\Phi$ does not involve any random variable, then $\mathbf{1}_{\Phi}$ can be deemed as a constant whose value depends only on whether $\Phi$ holds or not.

\noindent{\bf Filtrations and Stopping Times.} A \emph{filtration} of a probability space $(\Omega,\mathcal{F},\probm)$ is an infinite sequence $\{\mathcal{F}_n \}_{n\in\Nset_0}$ of $\sigma$-algebras over $\Omega$ such that $\mathcal{F}_n \subseteq \mathcal{F}_{n+1} \subseteq\mathcal{F}$ for all $n\in\Nset_0$.
A \emph{stopping time} (from $(\Omega,\mathcal{F},\probm)$) w.r.t $\{\mathcal{F}_n\}_{n\in\Nset_0}$ is a random variable $R:\Omega\rightarrow \Nset_0\cup\{\infty\}$ such that for every $n\in\Nset_0$, the event $R\le n$ belongs to $\mathcal{F}_n$.



%\noindent{\bf Conditional Variance.}
%Let $X$ be a bounded random variable (from some probability space).
%such that $\expv(|X|)<\infty$ and $\expv\left({\left(X-\condexpv{X}{\mathcal{G}}\right)}^2\right)<\infty$.
%The \emph{conditional variance} $\condvar{X}{\mathcal{G}}$ (cf.~\cite{ColinMcDiarmid1998concentration}) of $X$ given a sub-$\sigma$-algebra $\mathcal{G}$ is defined by
%$\condvar{X}{\mathcal{G}}:=\condexpv{{\left(X-\condexpv{X}{\mathcal{G}}\right)}^2}{\mathcal{G}}$\enskip.



\noindent{\bf (Conditionally) Difference-boundedness.}
A discrete-time stochastic process $\Gamma=\{X_n\}_{n\in\Nset_0}$ when adapted to a filtration $\{\mathcal{F}_n\}_{n\in\Nset_0}$, is
\begin{compactitem}
\item \emph{conditionally difference-bounded}, if there exists $c\in(0,\infty)$ such that for all $n\in\Nset_0$, we have $\expv\left(|X_{n+1}-X_n|\right)< \infty$, $\condexpv{|X_{n+1}-X_n|}{\mathcal{F}_n}\le c$ a.s.;
\item \emph{difference-bounded}, if there is $c\in(0,\infty)$ such that for every $n\in\Nset_0$, we have $|X_{n+1}-X_n|\le c$ a.s.
\end{compactitem}

\noindent{\bf Stopping time $\stopping{\Gamma}$.}
Given a discrete-time stochastic process $\Gamma=\{X_n\}_{n\in\Nset_0}$ adapted to a filtration $\{\mathcal{F}_n\}_{n\in\Nset_0}$, we define the random variable $\stopping{\Gamma}$ by
$\stopping{\Gamma}(\omega):=\min\{n\mid X_{n}(\omega)\le 0\}$
where $\min\emptyset:=\infty$.
%Moreover, we say that $\Gamma$ is \emph{stopped} if it holds for all sample points $\omega$ that for all $n\in\Nset_0$, $X_n(\omega)\le 0$ implies $X_{n+1}(\omega)=X_n(\omega)$.
Note that by definition, $\stopping{\Gamma}$ is a stopping time w.r.t $\{\mathcal{F}_n\}_{n\in\Nset_0}$.
Moreover,
\begin{eqnarray*}
\expv(\stopping{\Gamma}) &=& \infty\cdot \probm(\stopping{\Gamma}=\infty)+\sum_{k=0}^\infty k\cdot \probm(\stopping{\Gamma}=k)  \\
&=& \infty\cdot \probm(\stopping{\Gamma}=\infty)+\sum_{k=0}^\infty \probm(k<\stopping{\Gamma}<\infty)\enskip.
\end{eqnarray*}
We follow the convention that $0\cdot\infty:=0$ as in the setting of Lebesgue Integral.

\noindent{\bf Martingales.} A discrete-time stochastic process $\Gamma=\{X_n\}_{n\in\Nset}$ adapted to a filtration $\{\mathcal{F}_n\}_{n\in\Nset_0}$ is a \emph{martingale} (resp. \emph{supermartingale}, \emph{submartingale})
if for every $n\in\Nset_0$, $\expv(|X_n|)<\infty$ and it holds a.s. that
$\condexpv{X_{n+1}}{\mathcal{F}_n}=X_n$ (\mbox{resp. } $\condexpv{X_{n+1}}{\mathcal{F}_n}\le X_n$, $\condexpv{X_{n+1}}{\mathcal{F}_n}\ge X_n$).
We refer to ~\cite[Chapter~10]{probabilitycambridge} for more details.


